FP-Prune: Rethinking Visual Token Pruning from an Information Gain Perspective

Visual token pruning can reduce the inference cost of vision language models, but its effectiveness depends on preserving complementary visual information under a limited token budget. A central challenge is to quantify the additional information a candidate token contributes beyond the retained set, a contribution that conventional scores based on attention or similarity struggle to capture directly. In this work, we revisit visual token pruning from the perspective of information gain and use mutual information to characterize the incremental value of candidate tokens. We further establish theoretically that frame potential serves as an effective surrogate for mutual information. Building on this observation, we propose FP-Prune, a training-free visual token pruning method that iteratively removes tokens with low information gain to preserve as much complementary visual information as possible. Experiments on three widely used VLMs and eight datasets demonstrate that FP-Prune outperforms baseline methods in both accuracy and inference efficiency. Further analysis shows that the surrogate objective closely aligns with model performance. Our work provides theoretical grounding and an effective method for visual token pruning.

==> fp_text_spacing.tex <==
% Main-paper spacing only.
\makeatletter

% Spacing before run-in paragraph headings.
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
  {6pt}{-1em}{\normalfont\normalsize\bfseries}}

\makeatother

% Display-math spacing.
\newcommand{\FPDisplaySpacing}{%
  \setlength{\abovedisplayskip}{8pt}%
  \setlength{\belowdisplayskip}{8pt}%
  \setlength{\abovedisplayshortskip}{5pt}%
  \setlength{\belowdisplayshortskip}{8pt}%
}

\apptocmd{\normalsize}{\FPDisplaySpacing}{}{}
\AtBeginDocument{\FPDisplaySpacing}

\setlength{\intextsep}{10pt}
\setlength{\floatsep}{10pt}
\setlength{\dblfloatsep}{10pt}

% Short cross-reference paragraph.
\newcommand{\FPShortParagraph}[1]{{\raggedright #1\par}}

% Related Work heading.
\makeatletter

\newcommand{\FPRelatedWorkHeading}{%
  \let\FP@savedsection\cvprsection
  \def\cvprsection{\@startsection{section}{1}{\z@}%
    {-12pt plus -1pt minus -1pt}{9pt}{\large\bf}}%
  \section{Related Work}%
  \let\cvprsection\FP@savedsection
}

\makeatother

% Local spacing below Equation (12).
\newcommand{\FPCompactDisplayBelow}{%
  \setlength{\belowdisplayskip}{6pt}%
  \setlength{\belowdisplayshortskip}{6pt}%
}

